Locally Aggregated Feature Attribution on Natural Language Model Understanding

With the growing popularity of deep-learning models, model understanding becomes more important. Much effort has been devoted to demystify deep neural networks for better interpretability. Some feature attribution methods have shown promising results in computer vision, especially the gradient-based methods where effectively smoothing the gradients with reference data is key to a robust and faithful result. However, direct application of these gradient-based methods to NLP tasks is not trivial due to the fact that the input consists of discrete tokens and the "reference" tokens are not explicitly defined. In this work, we propose Locally Aggregated Feature Attribution (LAFA), a novel gradient-based feature attribution method for NLP models. Instead of relying on obscure reference tokens, it smooths gradients by aggregating similar reference texts derived from language model embeddings. For evaluation purpose, we also design experiments on different NLP tasks including Entity Recognition and Sentiment Analysis on public datasets as well as key feature detection on a constructed Amazon catalogue dataset. The superior performance of the proposed method is demonstrated through experiments.

==> Sec_Z_backup.tex <==
\section{Appendix : Ablation Study on Kernel Function}\label{appendix:A}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\textwidth]{Fig_kernel.png}
%  \caption{Comparisons for different kernel functions}
%  \label{fig:case_study4}
% \end{figure}

% The result is shown in Figure \ref{fig:case_study4}.
% From the result, we can observe that no single kernel function outperforms all other kernel functions under different mask ratios.
% Indicator kernel shows a good performance when the masked ratio is greater than $10\%$, while RBF kernel shows a good performance when the masked ratio is smaller than $5\%$. 
% Therefore, the choice of kernel depends on different use cases.

The kernel function $k(\cdot,\cdot)$ in Equation \eqref{eq:kernel_form} plays an important role in aggregation step.
We conduct ablation study on different choices of kernel functions, including Radial basis function kernel (\textit{RBF}), Cubic kernel (\textit{Cubic}), Laplacian kernel (\textit{Laplacian}), L2 norm (\textit{L2}) and Indicator function (\textit{Indicator}) under the position-level evaluation task. 
Due to the page limit, the details of kernel functions are listed in Subsection \ref{appendix: kernels}.
The results are shown in Figure \ref{fig:case_study_kernel_ablation}.
From the result, we observe that no single kernel function outperforms all other kernel functions under different mask ratios.
Indicator function shows a good performance when the masked ratio is greater than $10\%$, while RBF kernel shows a good performance when the masked ratio is smaller than $5\%$. 
To illustrate the intuition about different kernels, let's take the example in Figure \ref{fig:illustration} again.
If we use the indicator function as kernel, the brand "FakeBrand" can be smoothed only if the brand "FakeBrand"  appeared in the neighbors $\mathcal{X}_{sim}$. 
In other word, when "FakeBrand" is considered as important feature in the neighbors, the feature score of "FakeBrand" in original text would increase.
Suppose, in a pre-trained word embedding space, brand "FakeBrand" is close other brands. 
If we adopt non-indicator kernel, important brands highlighted by the neighbors can increase the feature score of "FakeBrand" in the original text as well based on Equation \eqref{eq:kernel_form}.
Therefore, the choice of kernel is flexible and depends on different use cases.


\begin{figure*}
  \centering
  \includegraphics[width=0.8\textwidth]{Fig_kernel.png}
 \caption{Comparisons for different kernel functions in Case III.}
 \label{fig:case_study_kernel_ablation}
\end{figure*}

\subsection{Kernel Choices}\label{appendix: kernels}

\begin{enumerate}
    \item Radial basis function kernel (\textit{RBF}) :
    \begin{equation*}
        k_{RBF}(a,b) = exp(-||a - b||_2 / l ^ 2),
    \end{equation*}
    where larger hyper-parameter $l$ indicates lower impact from neighbors and vice versa. In the numerical study, we choose $l = 2$ based on the range of embedding $a$ and $b$.
    \item Cubic kernel (\textit{Cubic}):
    \begin{equation*}
        k_{Cubic}(a,b) = (\gamma a^T b + c_0)^d,
    \end{equation*}
    where $\gamma = 7$, $c_0 = 0$ and $d = 3$, smaller $\gamma$ means lower impact from neighbors.
    \item Cosine kernel  (\textit{Cosine}):
    \begin{equation*}
        k_{Cos}(a,b) = a^T b/ ||a|||b|||
    \end{equation*}
    \item Laplacian kernel (\textit{Laplacian}):
    \begin{equation*}
        k_{Laplacian}(a,b) = exp(-||a - b||_1 / l ^ 2),
    \end{equation*}
    in the numerical study, we choose $l = 2$.
    \item L2 norm based similarity (\textit{L2}):
    \begin{equation*}
        k_{L2}(a,b) = 1/clip(||a - b||_2, \lambda_{left}, \lambda_{right}),
    \end{equation*}
    where $clip(\cdot, \lambda_{left}, \lambda_{right})$ denotes clip function with $\lambda_{left} = 0.3$ and $\lambda_{right} = 3$ as clip boundary in numerical study.
    \item Indicator function based similarity (\textit{Indicator}):
    \begin{equation*}
        k_{Indicator}(a,b) = \mathbb{I}(a, b),
    \end{equation*}
    where $\mathbb{I}(\cdot, \cdot)$ denotes indicator function.
\end{enumerate}



\section{Appendix : Neighbor Search Experiment based on SST}\label{appendix:B}
To clarify the neighbor searching process and the difference in result using different layers, we show some experiment below.

\subsection{Directly using the Glove Embedding}
Generally speaking, we can directly use the Glove embedding as the encoder, which is the input of BERT-based models and enable us to find neighbor in sense of "word similarity". However, sentence shares high similarity have totally opposite meanings. For instance, two sentences like "I do not \textbf{actually love} this movie because of some flaws" and "I like the movie \textbf{love actually}" both have two words in common but in the second one it is just a movie name, but not a sentiment factor. We argue that we can use some external label to make the layer selection as a supervise problem. Said we can maximize the average probability that a sentence's neighbor shares the same label. In such way we can find the neighbor in ways other than merely "word similarity".

\subsection{Layer selection supervised by sentence sentiment}
In this experiment, we uses the sentiment label itself as the rule to find a best layer for neighbor searching.

We randomly select $5000$ sentence pairs in the SST training or validation set, then we save the L-2 distance between two sentences in pooling average and categories them into two cases: same or different, which indicates if these two sentences share a same over-all sentiment label. The goal of this experiment is somewhat visualize the inner mechanic of selecting different layers as the encoder.

\begin{figure}
  \centering
  \includegraphics[width=0.4\textwidth]{Fig_bert_emb_nei.png}
 \caption{To be revised}
 \label{fig:app_sst_1}
\end{figure}

For example, as we can find in the figure \ref{fig:app_sst_1}, the final layer of DistilBERT model fine-tuned on the SST-2 classifies the distance of sentences into two batches, one of the same label and one for the opposite label. Such effect only exist in the layer seven, and the layer six somewhat have some discrimination of these two cases, but two curve shares a common area in considerable proportion. Layers one to five, however, cannot separate these two cases.

As a result, if we want to find sentence neighbor in the sense of "sentence sentiment", then the layer seven would be chosen as the encoder.

\subsection{Layer selection supervised by the factor model}
Owing to the fact that another gold label set is unavailable in the SST. We tried several set of labels generated by the topic model and want to select layers in the sense of the same topic \textbf{cite paper}.

Noted that this is more like a exploratory experiment so we do not tune the topic model but put all parameters as default. Seven sets of topic labels are being generated by the package \textbf{cite gensim} ranges from $3$ to $10$ topics.

The basic settings are the same as case study III. Said we grab a sentence, find its neighbors using different layers and find the precision scores (the same as the probability in the last case but we have more than two class here) of the labels of neighbor sentences. The experiment in this subsection is conducted on the first $100$ SST sentences in the training set.

\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{app_sst_2.png}
 \caption{To be revised}
 \label{fig:app_sst_2}
\end{figure}

The result are showing in figure \ref{fig:app_sst_2}. The layer that maximizes the topic precision for $3$ topics to $10$ topics are $4, 3, 4, 1, 1, 2, 3, 1$ respectively. We can see that as the number of topics growing, the Glove embedding itself contains enough information to separate different categories, or intuitively we are more likely to look into the "word similarity", but when topic number ranges from three to five, the middle layer has better discrimination of different clusters.

As a result, if we want to find sentence neighbor in the sense of "topic similarity", then the first several layers can be served as the encoder.

\subsection{DistilBERT performance on SST}
Here we fixed the max number of neighbors as $10$ and uses $0.05$ as the cut-off rate to filter those neighbors that are not "actually close". Given experiments showing above, we tried some layers selected by different methods. Layer $1$, $3$, $4$, and $7$ are chosen. We use the Simple Gradient and the Smooth Gradient as the baseline for comparison.

\begin{table}[H]
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cc}
\hline
                 & \multicolumn{2}{c}{Correlation}  \\ \cline{2-3} 
Method           &   SST2         &  SST+     \\ \hline
SimpleGrad        &   0.441(0.083) & 0.374(0.067)      \\
SpG + LAFA + L0   &   0.450(0.081) & 0.383(0.066)      \\
SpG + LAFA + L1   &   0.452(0.080) & 0.384(0.066)      \\
SpG + LAFA + L2   &   0.452(0.080) & 0.385(0.065)      \\
SpG + LAFA + L3   &   0.453(0.080) & 0.386(0.065)      \\
SpG + LAFA + L4   &   \textbf{0.453(0.080)} & \textbf{0.387(0.065)}      \\
SpG + LAFA + L5   &   0.453(0.080) & 0.384(0.065)      \\
SpG + LAFA + L6   &   0.449(0.082) & 0.378(0.067)      \\ \hline
SmoothGrad        &   0.484(0.073) & 0.407(0.068)      \\
SmG + LAFA + L0   &   0.494(0.071) & 0.416(0.067)      \\ 
SmG + LAFA + L1   & & \\ 
SmG + LAFA + L2   &   0.493(0.071) & 0.413(0.065)      \\ 
SmG + LAFA + L3   &   &      \\ 
SmG + LAFA + L4   & & \\
SmG + LAFA + L5   & & \\
SmG + LAFA + L6   &   &      \\\hline
\end{tabular}
}
\caption{Feature Attribution Result on SST.}
\label{table:app_sst_3}
\end{table}

From table \ref{table:app_sst_3} we can find out that LAFA is a generally good method that always beats the baseline in this setting once we use information from faithful neighbors. Among them the setting of \textbf{what} has the best performance.

\subsection{Effect of the number of neighbors in SST}
\textbf{pass}, or we could do cut off vs no cut off.

%We still advice to choose sentence neighbors carefully and 


\section{Appendix: Examples of different Feature Attribution Methods}


\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{Fig_case_re.png}
 \caption{Case Study for RE}
 \label{fig:case_study1_re}
\end{figure}



\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{Fig_case_2.png}
 \caption{Case Study for positional-level and word-level evaluation tasks. Green star indicates the "i5" in the description gets high feature attribution score after masking the "i5" in the tile.}
 \label{fig:case_study2}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{Fig_case_3.png}
 \caption{Case Study of feature attribution methods}
 \label{fig:case_study3}
\end{figure}
